Adapt-$\infty$: Scalable Continual Multimodal Instruction Tuning via Dynamic Data Selection

Visual instruction datasets from various distributors are released at different times and often contain a significant number of semantically redundant text-image pairs, depending on their task compositions (i.e., skills) or reference sources. This redundancy greatly limits the efficient deployment of continually adaptable multimodal large language models, hindering their ability to refine existing skills and acquire new competencies over time. We reframe the problem of lifelong Instruction Tuning (LiIT) via data selection, where the model automatically selects beneficial samples to learn from earlier and new datasets based on the current state of acquired knowledge in the model. We propose Adapt-$\infty$, a new multi-way and adaptive data selection approach that dynamically balances sample efficiency and effectiveness during LiIT. We first construct pseudo-skill clusters by grouping gradient-based sample vectors. Next, we select the best-performing data selector for each skill cluster from a pool of selector experts, including our newly proposed scoring function, Image Grounding score. This data selector samples a subset of the most important samples from each skill cluster for training. To prevent the continuous increase in the size of the dataset pool during LiIT, we introduce a cluster-wise permanent data pruning strategy to remove the most semantically redundant samples from each cluster, keeping computational requirements manageable. We validate the effectiveness and efficiency of Adapt-$\infty$ over a sequence of multimodal instruction tuning datasets with various tasks, including (Knowledge) VQA, multilingual, grounding, reasoning, language-only, and multi-image comprehension. Training with samples selected by Adapt-$\infty$ alleviates catastrophic forgetting, especially for rare tasks, and promotes forward transfer across the continuum using only a fraction of the original data.

==> materials/fig_ccs_ppl.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/ccs_ppl.png}
    \caption{Distribution of perplexity scores in various multimodal instruction tuning datasets and the placement of CCS bins \citep{zheng2023coverage} over the respective ranges. The perplexity scores are extracted using the LLaVA 1.5 multimodal LLM \citep{liu2023improved}.}
    \label{fig:ccs_ppl}
\end{figure}

==> materials/fig_dist_analysis.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/m3it_hit.png}
    \caption{Comparison of score histograms across task categories in the M3IT instruction dataset \citep{li2023m}. The scoring functions are perplexity (left) and image-grounding (right). \jy{quick question; the range of x and y axis is different. I guess x is due to the metric differences}}
    \label{fig:m3it_hist}
\end{figure}
